BASED-XAI: Breaking Ablation Studies Down for Explainable Artificial Intelligence

Explainable artificial intelligence (XAI) methods lack ground truth. In its place, method developers have relied on axioms to determine desirable properties for their explanations' behavior. For high stakes uses of machine learning that require explainability, it is not sufficient to rely on axioms as the implementation, or its usage, can fail to live up to the ideal. As a result, there exists active research on validating the performance of XAI methods. The need for validation is especially magnified in domains with a reliance on XAI. A procedure frequently used to assess their utility, and to some extent their fidelity, is an ablation study. By perturbing the input variables in rank order of importance, the goal is to assess the sensitivity of the model's performance. Perturbing important variables should correlate with larger decreases in measures of model capability than perturbing less important features. While the intent is clear, the actual implementation details have not been studied rigorously for tabular data. Using five datasets, three XAI methods, four baselines, and three perturbations, we aim to show 1) how varying perturbations and adding simple guardrails can help to avoid potentially flawed conclusions, 2) how treatment of categorical variables is an important consideration in both post-hoc explainability and ablation studies, and 3) how to identify useful baselines for XAI methods and viable perturbations for ablation studies.

==> 06_TODO.tex <==
% \section{TODO}
% \begin{itemize}
    % \item Run all global exps
        % \begin{todolist}
            % \item  add plots to Subsection 4.1
            % \item  add analysis to Subsection 4.1  (at least visual/trends, point out interesting differences in behavior)
        % \end{todolist}
    % \item Run all local exps
        % \begin{todolist}
            % \item  add plots to Subsection 4.2
            % \item  add analysis to Subsection 4.2  
        % \end{todolist}
    % \item Add \textit{guardrails} to analysis
        %  \begin{todolist}
            %   \item  add noisy / uninformative features
            %   \item  train naive/baseline/worst case model and performance metrics (how do we add it to plots...)
        % \end{todolist}
    % \item Do we have sufficient baselines and perturbations?  Survey literature to find additional - or determine completeness.  
        % \begin{todolist}
            % \item  Use references of papers that we have read and arxiv's connected paper function (shows network of connected papers)
            % \item  Summarizing findings in Previous work section and add referecences to ablation.bib  
        % \end{todolist}
    % \item Rank order of feature importance (local, global), spambase, adult, german
        .  

% \end{itemize}

% \pagebreak
\listoftodos

==> old/03_method_messed_up.tex <==
\section{Method}
\begin{figure*}[h]
  \includegraphics[width=0.9\textwidth]{figures/section_3/diagram.png}
  \caption{Diagram of data and logic flow for an ablation study.}
  \label{fig:adult_global}
\end{figure*}


\subsection{Overview}
In this section we describe the process of an ablation study  
given a trained model $f:\cX \to \cY$, where $\cX = \R^(n x d)$ and $\cY = \R^d$. The following can also be generalized for multi-class classification problems. We refer to single inputs $x_i \in \cX \; \forall i \in \{1\dots n\}$ and their features as $x^j \; \forall j \in \{1\dots d\}$. 

An ablation study relies on perturbations and explanation methods. 
\begin{dfn}
    A perturbation $p \sim \cP$ attempts to remove information from $x_i^j$ by replacing $x_i^j$ with $p_i^j$. 
\end{dfn}

\begin{dfn}
    An explanation method is any local feature attribution or global importance method $A$ that attributes the output of $f$ for a specific observation $x_i$ or assign importance to each feature for a collection of observations. 
\end{dfn}

There are a wide variety of explanation methods that exist. We use methods in our evaluation which require baseline distributions. 

\begin{dfn}
    Baselines are reference distributions used in general removal or gradient based explanation methods. Baselines can be default values or a distribution over which removed features are marginalized. 
\end{dfn}

\begin{dfn}
    An ablation study attempts to assess the validity of local or global explanation methods through examining relative model performance change after perturbing input features $x^j$ in order of importance. 
\end{dfn}

\subsection{Ablation Study Algorithm}

We detail the steps of an ablation study in Algorithm \ref{alg:ablation}. Ideally ablation studies expect that any good explanation method will return explanation values that adhere to the following property: Features removed from the model with higher importances decrease model performance more than those with lower importances.

\begin{algorithm}
\caption{Ablation study}
\label{alg:ablation}
\begin{algorithmic}[1]
\State Given a model $f$, evaluation data $X, Y$, perturbation distribution $\cP$, baseline distribution $\cB$, explanation method $A(X, f, b)$, and accuracy or loss metric $\cL$.
\State Initialize $scores$ to track loss metric
\For{t $\leftarrow  1 \dots T$}
\State Sample $b \sim \cB$ and $p \sim \cP$.
\For{$i \leftarrow \{1 \dots n\}$}
\State Compute explanations $e_i$ via method $A$ and baseline $b$ 
\State Compute ranking $r_i \leftarrow argsort(e_i)$ in decreasing order where $r_i^k$ is index of the $k$th ranked feature.
\EndFor
\State $scores(t, 0) \leftarrow  \cL(f(X),Y)$ \Comment{Loss on original $X$}
\For{$k \leftarrow \{1 \dots d\}$} 
\For{$i \leftarrow \{1 \dots n\}$}
\State $m \leftarrow r_i^k$  \Comment{$k$th ranked feature for $x_i$}
\State $x_i^{m} \leftarrow p_i^{m}$ \Comment{perturb $x_i$}
\EndFor
\State $scores(t, k) \leftarrow \cL(f(X),Y)$
\EndFor
\EndFor
\State \Return scores
\end{algorithmic}
\end{algorithm}



\subsection{Baseline and Perturbation Distributions}
Using the following set of  marginal distributions as either perturbations during ablation, or as background/baseline samples:

\begin{table}[ht!] 
    \begin{tabular}{|c||c|c|c|}
    % { | m{3cm} | m{1cm}| m{1cm} | m{3cm}} 
    \hline
    Distribution      & Perturbation      & Baseline   & Reference \\
    % \midrule
    \hline
    constant median   & \checkmark    & \checkmark  &   \\ 
    marginal          & \checkmark    &             & \cite{breiman2001}                            \\
    nearest neighbors &               & \checkmark  &  \cite{albini2021counterfactual}\\              
    opposite class    &               & \checkmark  &    \cite{albini2021counterfactual}\\      
    training          &               & \checkmark  &  \cite{lundberg2017unified,haug2021baselines}   \\
    max distance      & \checkmark    &   & \cite{haug2021baselines,sturmfels2020visualizing} \\
    \hline
    \end{tabular}    
\caption{\label{tab:perturb_baseline}List of marginal distributions used in ablation studies and as baselines for local attributions.}
\end{table}

The \textit{constant median} distribution is a variant of the constant distribution which is simply the median of each feature. We believe this is a more meaningful baseline than a constant zero baseline for tabular data. 

We use the \textit{marginal} distribution as a perturbation  replacing each perturbed feature with a random value in the training marginal distribution of that feature. [comment on source of this distribution]

The \textit{training} baseline also known as the expectation baseline is a sub-sample of the training data \cite{lundberg2017unified}. 

We borrow two baselines from \citet{albini2021counterfactual} that introduce alternative counterfactual baselines. The \textit{opposite class} baseline includes a sample of observations from the training data with an observed class that is opposite of the predicted class of the explained observation. 

Finally, we re-purpose the \textit{max distance} distribution from \citet{sturmfels2020visualizing} as a perturbation method [insert why].

\subsection{Models}

We train differentiable models for each ablation study to expand our set of available explanation methods. We train a two layer neural network with hidden neurons proportional to the number of features in each dataset. We select the best performing model with early stopping on held out validation data. 

\subsection{Explanation Methods}

We use three different explanation methods in our ablation studies. These methods include model agnostic, gradient based, and Shapley value based methods. 

\begin{itemize}
    \item DeepShap (DS) [cite]
    \item Integrated Gradients (IG) [cite]
    \item KernelShap (KS) [cite]
\end{itemize}

We use each of these methods to generate local explanations. Global explanations are simply the average absolute value across all observations in the dataset.

\subsection{Categorical Treatment}

We explore using proper treatments for categorical variables. Previous work often does not address tabular data [cite?], and when it does, categorical variables do not have their own distributional assumptions in explanations or perturbations. We propose two alterations to the ablation process in the presence of categorical variables. 
\begin{enumerate}
    \item We rank of explanations on an individual feature level. Each categorical variable has a single ranking that we derive from the sum of attributions of their onehot features. 
    \item We perform perturbations on an individual feature level. Any perturbations to categorical variables result in a category from the training distribution.
\end{enumerate}

Performing perturbations in the multinomial category space is feasible for a majority of our perturbation distributions, however we need to alter \textit{constant median} and \textit{max distance}. We define \textit{constant median} for categorical variables as the most common category. Since \textit{max distance} in continuous space is the furthest point in $L_1$ space, we propose sampling uniformly from the other categories. Formally, we create the perturbation distribution for a categorical feature $x_i^j = a$ with categories $C$ as: 
$$\cP = \{c | c \in C, \; c \neq a\}$$







% \subsection{MISC SCRATCH SPACE}
% Questions raised by our definition the we need to be able to answer:
% \begin{enumerate}
%     \item How do we evaluate if we have minimized a feature's importance? Or phrased another way - what makes a good ablation method?
%     \begin{itemize}
%         \item Is rerunning the predictions on the dataset with the ablated feature sufficient?  
%         \item If we normalized the global importances so they summed to one, is the best ablation method the one that drops model performance in proportion to the feature importance?
%         \item What if we find a method that drops model performance further than expected?  Is that a better ablation method or a bad set of explanations?
%     \end{itemize}   
    
%     \item Should it be just one feature at a time?  In the presence of correlated variables - would ablating principal components be "better"?
%     \item \sout{Should we retrain the model having dropped it entirely?  (this would be an improvement on ROAR...which ablated pixels, but never tested their assumption that the ablated pixels had no importance)} - a good question to answer, but probably not in a workshop paper - will add in for a conference paper
% \end{enumerate}


\subsection{Insights}

We discussed putting in informative insights that help change thinking from images to tabular:
\begin{itemize}
    \item Min is the same as 0 baseline for images
    \item What can and can't be used as perturbation vs baseline?
\end{itemize}

\section{Method}
\begin{figure*}[h]
  \includegraphics[width=0.9\textwidth]{figures/section_3/diagram.png}
  \caption{Diagram of data and logic flow for an ablation study.}
  \label{fig:adult_global}
\end{figure*}





\subsection{Baseline and Perturbation Distributions}
Using the following set of  marginal distributions as either perturbations during ablation, or as background/baseline samples:

\begin{table}[ht!] 
    \begin{tabular}{|c||c|c|c|}
    % { | m{3cm} | m{1cm}| m{1cm} | m{3cm}} 
    \hline
    Distribution      & Perturbation      & Baseline   & Reference \\
    % \midrule
    \hline
    constant median   & \checkmark    & \checkmark  &   \\ 
    marginal          & \checkmark    &             & \cite{breiman2001}                            \\
    nearest neighbors &               & \checkmark  &  \cite{albini2021counterfactual}\\              
    opposite class    &               & \checkmark  &    \cite{albini2021counterfactual}\\      
    training          &               & \checkmark  &  \cite{lundberg2017unified,haug2021baselines}   \\
    max distance      & \checkmark    &   & \cite{haug2021baselines,sturmfels2020visualizing} \\
    \hline
    \end{tabular}    
\caption{\label{tab:perturb_baseline}List of marginal distributions used in ablation studies and as baselines for local attributions.}
\end{table}

The \textit{constant median} distribution is a variant of the constant distribution which is simply the median of each feature. We believe this is a more meaningful baseline than a constant zero baseline for tabular data. 

We use the \textit{marginal} distribution as a perturbation  replacing each perturbed feature with a random value in the training marginal distribution of that feature. [comment on source of this distribution]

The \textit{training} baseline also known as the expectation baseline is a sub-sample of the training data \cite{lundberg2017unified}. 

We borrow two baselines from \citet{albini2021counterfactual} that introduce alternative counterfactual baselines. The \textit{opposite class} baseline includes a sample of observations from the training data with an observed class that is opposite of the predicted class of the explained observation. 

Finally, we re-purpose the \textit{max distance} distribution from \citet{sturmfels2020visualizing} as a perturbation method [insert why].

\subsection{Models}

We train differentiable models for each ablation study to expand our set of available explanation methods. We train a two layer neural network with hidden neurons proportional to the number of features in each dataset. We select the best performing model with early stopping on held out validation data. 

\subsection{Explanation Methods}

We use three different explanation methods in our ablation studies. These methods include model agnostic, gradient based, and Shapley value based methods. 

\begin{itemize}
    \item DeepShap (DS) [cite]
    \item Integrated Gradients (IG) [cite]
    \item KernelShap (KS) [cite]
\end{itemize}

We use each of these methods to generate local explanations. Global explanations are simply the average absolute value across all observations in the dataset.

\subsection{Categorical Treatment}

We explore using proper treatments for categorical variables. Previous work often does not address tabular data [cite?], and when it does, categorical variables do not have their own distributional assumptions in explanations or perturbations. We propose two alterations to the ablation process in the presence of categorical variables. 
\begin{enumerate}
    \item We rank of explanations on an individual feature level. Each categorical variable has a single ranking that we derive from the sum of attributions of their onehot features. 
    \item We perform perturbations on an individual feature level. Any perturbations to categorical variables result in a category from the training distribution.
\end{enumerate}

Performing perturbations in the multinomial category space is feasible for a majority of our perturbation distributions, however we need to alter \textit{constant median} and \textit{max distance}. We define \textit{constant median} for categorical variables as the most common category. Since \textit{max distance} in continuous space is the furthest point in $L_1$ space, we propose sampling uniformly from the other categories. Formally, we create the perturbation distribution for a categorical feature $x_i^j = a$ with categories $C$ as: 
$$\cP = \{c | c \in C, \; c \neq a\}$$







% \subsection{MISC SCRATCH SPACE}
% Questions raised by our definition the we need to be able to answer:
% \begin{enumerate}
%     \item How do we evaluate if we have minimized a feature's importance? Or phrased another way - what makes a good ablation method?
%     \begin{itemize}
%         \item Is rerunning the predictions on the dataset with the ablated feature sufficient?  
%         \item If we normalized the global importances so they summed to one, is the best ablation method the one that drops model performance in proportion to the feature importance?
%         \item What if we find a method that drops model performance further than expected?  Is that a better ablation method or a bad set of explanations?
%     \end{itemize}   
    
%     \item Should it be just one feature at a time?  In the presence of correlated variables - would ablating principal components be "better"?
%     \item \sout{Should we retrain the model having dropped it entirely?  (this would be an improvement on ROAR...which ablated pixels, but never tested their assumption that the ablated pixels had no importance)} - a good question to answer, but probably not in a workshop paper - will add in for a conference paper
% \end{enumerate}


\subsection{Insights}

We discussed putting in informative insights that help change thinking from images to tabular:
\begin{itemize}
    \item Min is the same as 0 baseline for images
    \item What can and can't be used as perturbation vs baseline?
\end{itemize}





\subsection{Baseline and Perturbation Distributions}
Using the following set of  marginal distributions as either perturbations during ablation, or as background/baseline samples:

\begin{table}[ht!] 
    \begin{tabular}{|c||c|c|c|}
    % { | m{3cm} | m{1cm}| m{1cm} | m{3cm}} 
    \hline
    Distribution      & Perturbation      & Baseline   & Reference \\
    % \midrule
    \hline
    constant median   & \checkmark    & \checkmark  &   \\ 
    marginal          & \checkmark    &             & \cite{breiman2001}                            \\
    nearest neighbors &               & \checkmark  &  \cite{albini2021counterfactual}\\              
    opposite class    &               & \checkmark  &    \cite{albini2021counterfactual}\\      
    training          &               & \checkmark  &  \cite{lundberg2017unified,haug2021baselines}   \\
    max distance      & \checkmark    &   & \cite{haug2021baselines,sturmfels2020visualizing} \\
    \hline
    \end{tabular}    
\caption{\label{tab:perturb_baseline}List of marginal distributions used in ablation studies and as baselines for local attributions.}
\end{table}

The \textit{constant median} distribution is a variant of the constant distribution which is simply the median of each feature. We believe this is a more meaningful baseline than a constant zero baseline for tabular data. 

We use the \textit{marginal} distribution as a perturbation  replacing each perturbed feature with a random value in the training marginal distribution of that feature. [comment on source of this distribution]

The \textit{training} baseline also known as the expectation baseline is a sub-sample of the training data \cite{lundberg2017unified}. 

We borrow two baselines from \citet{albini2021counterfactual} that introduce alternative counterfactual baselines. The \textit{opposite class} baseline includes a sample of observations from the training data with an observed class that is opposite of the predicted class of the explained observation. 

Finally, we re-purpose the \textit{max distance} distribution from \citet{sturmfels2020visualizing} as a perturbation method [insert why].

\subsection{Models}

We train differentiable models for each ablation study to expand our set of available explanation methods. We train a two layer neural network with hidden neurons proportional to the number of features in each dataset. We select the best performing model with early stopping on held out validation data. 

\subsection{Explanation Methods}

We use three different explanation methods in our ablation studies. These methods include model agnostic, gradient based, and Shapley value based methods. 

\begin{itemize}
    \item DeepShap (DS) [cite]
    \item Integrated Gradients (IG) [cite]
    \item KernelShap (KS) [cite]
\end{itemize}

We use each of these methods to generate local explanations. Global explanations are simply the average absolute value across all observations in the dataset.

\subsection{Categorical Treatment}

We explore using proper treatments for categorical variables. Previous work often does not address tabular data [cite?], and when it does, categorical variables do not have their own distributional assumptions in explanations or perturbations. We propose two alterations to the ablation process in the presence of categorical variables. 
\begin{enumerate}
    \item We rank of explanations on an individual feature level. Each categorical variable has a single ranking that we derive from the sum of attributions of their onehot features. 
    \item We perform perturbations on an individual feature level. Any perturbations to categorical variables result in a category from the training distribution.
\end{enumerate}

Performing perturbations in the multinomial category space is feasible for a majority of our perturbation distributions, however we need to alter \textit{constant median} and \textit{max distance}. We define \textit{constant median} for categorical variables as the most common category. Since \textit{max distance} in continuous space is the furthest point in $L_1$ space, we propose sampling uniformly from the other categories. Formally, we create the perturbation distribution for a categorical feature $x_i^j = a$ with categories $C$ as: 
$$\cP = \{c | c \in C, \; c \neq a\}$$







% \subsection{MISC SCRATCH SPACE}
% Questions raised by our definition the we need to be able to answer:
% \begin{enumerate}
%     \item How do we evaluate if we have minimized a feature's importance? Or phrased another way - what makes a good ablation method?
%     \begin{itemize}
%         \item Is rerunning the predictions on the dataset with the ablated feature sufficient?  
%         \item If we normalized the global importances so they summed to one, is the best ablation method the one that drops model performance in proportion to the feature importance?
%         \item What if we find a method that drops model performance further than expected?  Is that a better ablation method or a bad set of explanations?
%     \end{itemize}   
    
%     \item Should it be just one feature at a time?  In the presence of correlated variables - would ablating principal components be "better"?
%     \item \sout{Should we retrain the model having dropped it entirely?  (this would be an improvement on ROAR...which ablated pixels, but never tested their assumption that the ablated pixels had no importance)} - a good question to answer, but probably not in a workshop paper - will add in for a conference paper
% \end{enumerate}


\subsection{Insights}

We discussed putting in informative insights that help change thinking from images to tabular:
\begin{itemize}
    \item Min is the same as 0 baseline for images
    \item What can and can't be used as perturbation vs baseline?
\end{itemize}


